Dark Energy Survey Year 1 Results: tomographic cross-correlations between DES galaxies and CMB lensing from SPT+Planck

We measure the cross-correlation between redMaGiC galaxies selected from the Dark Energy Survey (DES) Year-1 data and gravitational lensing of the cosmic microwave background (CMB) reconstructed from South Pole Telescope (SPT) and Planck data over 1289 sq. deg. When combining measurements across multiple galaxy redshift bins spanning the redshift range of $0.15<z<0.90$, we reject the hypothesis of no correlation at 19.9$\sigma$ significance. When removing small-scale data points where thermal Sunyaev-Zel'dovich signal and nonlinear galaxy bias could potentially bias our results, the detection significance is reduced to 9.9$\sigma$. We perform a joint analysis of galaxy-CMB lensing cross-correlations and galaxy clustering to constrain cosmology, finding $\Omega_{\rm m} = 0.276^{+0.029}_{-0.030}$ and $S_{8}=\sigma_{8}\sqrt{\mathstrut \Omega_{\rm m}/0.3} = 0.800^{+0.090}_{-0.094}$. We also perform two alternate analyses aimed at constraining only the growth rate of cosmic structure as a function of redshift, finding consistency with predictions from the concordance $\Lambda$CDM model. The measurements presented here are part of a joint cosmological analysis that combines galaxy clustering, galaxy lensing and CMB lensing using data from DES, SPT and Planck.

==> affiliations.tex <==
\section*{Affiliations}
\textit{
$^{1}$ Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94305\\ 
$^{2}$ Dept. of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305\\ 
$^{3}$ Department of Physics and McGill Space Institute, McGill University, Montreal, Quebec H3A 2T8, Canada\\ 
$^{4}$ Universit\"{a}ts-Sternwarte, Fakult\"{a}t f\"{u}r Physik, Ludwig Maximilians Universit\"{a}t M\"{u}nchen, Scheinerstr. 1, 81679 M\"{u}nchen, Germany\\ 
$^{5}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\ 
$^{6}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\ 
$^{7}$ Institute of Space Sciences (IEEC-CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\ 
$^{8}$ Center for Particle Cosmology, Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA,  USA 19104\\ 
$^{9}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{10}$ Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}ogicas(CIEMAT), Madrid, Spain\\ 
$^{11}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\ 
$^{12}$ Fermi National Accelerator Laboratory, MS209, P.O. Box 500, Batavia, IL 60510\\ 
$^{13}$ Department of Physics, University of Florida, Gainesville, Florida 32611, USA\\ 
$^{14}$ Institute of Physics, Laboratory of Astrophysics, \'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland\\ 
$^{15}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University,Columbus, OH 43210, USA\\ 
$^{16}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy\\ 
$^{17}$ High Energy Physics Division, Argonne National Laboratory, Argonne, IL, USA 60439\\ 
$^{18}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{19}$ Department of Physics and Astronomy, McMaster University, 1280 Main St. W., Hamilton, ON L8S 4L8, Canada\\ 
$^{20}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{21}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\ 
$^{22}$ Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721\\ 
$^{23}$ Jet Propulsion Laboratory, California Institute of Technology, Pasadena, CA 91109, USA\\ 
$^{24}$ Max-Planck-Institut f\"{u}r extraterrestrische Physik, 85748 Garching, Germany\\ 
$^{25}$ Faculty of Physics, Ludwig-Maximilians-Universit\"{a}t, 81679 M\"{u}nchen, Germany\\ 
$^{26}$ Einstein Fellow\\ 
$^{27}$ Astronomy Department, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\ 
$^{28}$ Department of Physics, University of Illinois Urbana-Champaign, 1110 W. Green Street, Urbana, IL 61801, USA\\ 
$^{29}$ Canadian Institute for Advanced Research, CIFAR Program in Cosmology and Gravity, Toronto, ON, M5G 1Z8, Canada\\ 
$^{30}$ Department of Physics, University of Michigan, Ann  Arbor, MI, USA 48109\\ 
$^{31}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\ 
$^{32}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\ 
$^{33}$ Institut de F\'{i}sica d`Altes Energies (IFAE), The Barcelona Instituteof Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\ 
$^{34}$ School of Physics, University of Melbourne, Parkville, VIC 3010, Australia\\ 
$^{35}$ SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025\\ 
$^{36}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\ 
$^{37}$ Department of Physics, University of Chicago, Chicago, IL, USA 60637\\ 
$^{38}$ Enrico Fermi Institute, University of Chicago, Chicago, IL, USA 60637\\ 
$^{39}$ California Institute of Technology, Pasadena, CA, USA 91125\\ 
$^{40}$ Department of Physics, University of California, Berkeley, CA, USA 94720\\ 
$^{41}$ Center for Astrophysics and Space Astronomy, Department of Astrophysical and Planetary Sciences, University of Colorado, Boulder, CO, 80309\\ 
$^{42}$ European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany\\ 
$^{43}$ Department of Physics, University of Colorado, Boulder, CO, 80309\\ 
$^{44}$ University of Chicago, Chicago, IL, USA 60637\\ 
$^{45}$ Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA, USA 94720\\ 
$^{46}$ Excellence Cluster Universe, 85748 Garching, Germany\\ 
$^{47}$ Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\ 
$^{48}$ Department of Physics, University of Minnesota, Minneapolis, MN, USA 55455\\ 
$^{49}$ Physics Department, Center for Education and Research in Cosmology and Astrophysics, Case Western Reserve University,Cleveland, OH, USA 44106\\ 
$^{50}$ Liberal Arts Department, School of the Art Institute of Chicago, Chicago, IL, USA 60603\\ 
$^{51}$ Harvard-Smithsonian Center for Astrophysics, Cambridge, MA, USA 02138\\ 
$^{52}$ Department of Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\ 
}

==> authorlist_backup.tex <==
%\author[T. Giannantonio, P. Fosalba et al.] {T.~Giannantonio$^{1,2,3}$\thanks{t.giannantonio@ast.cam.ac.uk}, P.~Fosalba$^{4 \thanks{fosalba@ice.cat}}$,
%B. Hoyle, D. Gruen, G. M. Bernstein, M. M. Rau, J. De Vicente, W. G. Hartley, E. Gaztanaga, J. DeRose, M. A. Troxel, C. Davis, A. Alarcon, N. MacCrann, J. Prat, C. Sánchez, E. Sheldon, R. H. Wechsler,

\def\KIPAC{1}
\def\Stanford{2}
\def\McGill{3}
\def\LMU{4}
\def\KICC{5}
\def\IoA{6}
\def\IEEC{7}
\def\Penn{8}
\def\KICP{9}
\def\CIEMAT{10}
\def\Portsmouth{11}
\def\FNAL{12}
\def\Florida{13}
\def\EPFL{14}
\def\CCAPP{15}
\def\Manchester{16}
\def\ArgonneHEP{17}
\def\KICPChicago{18}
\def\McMaster{19}
\def\AAUChicago{20}
\def\CMU{21}
\def\Arizona{22}
\def\JPL{23}
\def\MPE{24}
\def\Munich{25}
\def\Einstein{26}
\def\Illast{27}
\def\Illphys{28}
\def\Cifar{29}
\def\Michigan{30}
\def\UCL{31}
\def\OSU{32}
\def\IFAE{33}
\def\Melbourne{34}
\def\SLAC{35}
\def\Edinburgh{36}
\def\PhysicsUChicago{37}
\def\EFIChicago{38}
\def\Caltech{39}
\def\Berkeley{40}
\def\Colorado{41}
\def\ESO{42}
\def\Colphys{43}
\def\UChicago{44}
\def\LBNL{45}
\def\ExcellenceCluster{46}
\def\Dunlap{47}
\def\Minnesota{48}
\def\CaseWestern{49}
\def\ArtInstChicago{50}
\def\CfA{51}
\def\UToronto{52}

\author[Omori et al.] {
\parbox{\textwidth}{
Y.~Omori$^{\KIPAC,\Stanford,\McGill}$,
T.~Giannantonio$^{\LMU,\KICC,\IoA}$,
A.~Porredon$^{\IEEC}$,
E.~Baxter$^{\Penn}$,
C.~Chang$^{\KICP}$,
M.~Crocce$^{\IEEC}$,
P.~Fosalba$^{\IEEC}$,
A.~Alarcon$^{\IEEC}$,
S.~Avila$^{\CIEMAT,\Portsmouth}$,
N.~Banik$^{\FNAL,\Florida}$,
J.~Blazek$^{\EPFL,\CCAPP}$,
S.~L.~Bridle$^{\Manchester}$,
L.~E.~Bleem$^{\ArgonneHEP,\KICPChicago}$,
R.~Cawthon$^{\KICP}$,
A.~Drlica-Wagner$^{\FNAL}$,
A.~Choi$^{\CCAPP}$,
R.~Chown$^{\McGill,\McMaster}$,
T.~M.~Crawford$^{\KICPChicago,\AAUChicago}$,
S.~Dodelson$^{\CMU,\FNAL}$,
T.~F.~Eifler$^{\Arizona,\JPL}$,
J.~Elvin-Poole$^{\Manchester}$,
O.~Friedrich$^{\MPE,\Munich}$,
D.~Gruen$^{\KIPAC,\Stanford,\Einstein}$,
G.~P.~Holder$^{\Illast,\Illphys,\Cifar}$,
D.~Huterer$^{\Michigan}$,
B.~Jain$^{\Penn}$,
M.~Jarvis$^{\Penn}$,
D.~Kirk$^{\UCL}$,
N.~Kokron$^{\KIPAC,\Stanford}$,
E.~Krause$^{\Arizona,\JPL}$,
N.~MacCrann$^{\CCAPP,\OSU}$,
J.~Muir$^{\Michigan}$,
J.~Prat$^{\IFAE}$,
C.~L.~Reichardt$^{\Melbourne}$,
A.~J.~Ross$^{\CCAPP}$,
E.~Rozo$^{\Arizona}$,
E.~S.~Rykoff$^{\SLAC,\KIPAC}$,
C.~S{\'a}nchez$^{\Penn}$,
L.~F.~Secco$^{\Penn}$,
I.~Sevilla-Noarbe$^{\CIEMAT}$,
G.~Simard$^{\McGill}$,
M.~A.~Troxel$^{\CCAPP,\OSU}$,
R.~H.~Wechsler$^{\KIPAC,\Stanford,\SLAC}$,
J.~Zuntz$^{\Edinburgh}$,
J.~E.~Carlstrom$^{\KICPChicago,\PhysicsUChicago,\ArgonneHEP,\AAUChicago,\EFIChicago}$,
C.~L.~Chang$^{\ArgonneHEP,\KICPChicago,\AAUChicago}$,
H-M.~Cho$^{\SLAC}$,
A.~T.~Crites$^{\KICPChicago,\AAUChicago,\Caltech}$,
T.~de~Haan$^{\McGill,\Berkeley}$,
M.~A.~Dobbs$^{\McGill,\Cifar}$,
W.~B.~Everett$^{\Colorado}$,
E.~M.~George$^{\Berkeley,\ESO}$,
N.~W.~Halverson$^{\Colorado,\Colphys}$,
N.~L.~Harrington$^{\Berkeley}$,
W.~L.~Holzapfel$^{\Berkeley}$,
J.~D.~Hrubes$^{\UChicago}$,
A.~T.~Lee$^{\Berkeley,\LBNL}$,
E.~M.~Leitch$^{\KICPChicago,\AAUChicago}$,
D.~Luong-Van$^{\UChicago}$,
D.~P.~Marrone$^{\Arizona}$,
J.~J.~McMahon$^{\Michigan}$,
S.~S.~Meyer$^{\KICPChicago,\AAUChicago,\EFIChicago,\PhysicsUChicago}$,
L.~M.~Mocanu$^{\KICPChicago,\AAUChicago}$,
J.~J.~Mohr$^{\Munich,\ExcellenceCluster,\MPE}$,
T.~Natoli$^{\KICPChicago,\PhysicsUChicago,\Dunlap}$,
S.~Padin$^{\KICPChicago,\AAUChicago}$,
C.~Pryke$^{\Minnesota}$,
C.~L.~Reichardt$^{\Berkeley,\Melbourne}$,
J.~E.~Ruhl$^{\CaseWestern}$,
J.~T.~Sayre$^{\CaseWestern,\Colorado}$,
K.~K.~Schaffer$^{\KICPChicago,\EFIChicago,\ArtInstChicago}$,
E.~Shirokoff$^{\Berkeley,\KICPChicago,\AAUChicago}$, 
Z.~Staniszewski$^{\CaseWestern,\JPL}$,
A.~A.~Stark$^{\CfA}$,
K.~Vanderlinde$^{\Dunlap,\UToronto}$,
J.~D.~Vieira$^{\Illast,\Illphys}$, 
R.~Williamson$^{\KICPChicago,\AAUChicago}$,  +DES builders
}
\vspace{0.4cm} \\
\parbox{\textwidth}{Author affiliations are listed at the end of this paper}}



==> backup_text.tex <==
  %\textcolor{red}{EB: seems like we should take the GK approach of quoting a number without scale cuts} over five redshift bins spanning the photometric redshift range $\left[0.15-0.90\right]$  using conservative angular scale cuts motivated in \cite{Baxter2018} %\textcolor{blue}{ \sout{, and \postblinding{18.0$\sigma$} without these scale cuts}}.%suggestion by Troxel to remove S/N without scalecuts
  %\tg{Need to get single significance number from either fitting $\sigma_8$ from KN only, or from $\sqrt{D C^{-1} D}$}.  
%Under these scale cuts, we test for potential systematic contaminations and find no evidence of statistically significant biases in the cross-correlations.\textcolor{}} 
%given our fiducial choice of scale cuts. 
%The scale cuts were chosen to minimize the bias coming from residual thermal Sunyaev-Zel'dovich (tSZ) emission in the CMB temperature maps used to reconstruct the lensing map.  

%\begin{equation}
%\kappa_{\rm CMB} = \kappa^{true}_{\rm CMB} +  \kappa^{true}_{\mathcal{S}} + \kappa^{true}_{\rm tSZ}+ \kappa^{true}_{\rm CIB}
%\end{equation}

%The tSZ effect is caused by inverse Compton scattering of CMB photons with hot electrons.  At frequencies near 150 GHz, this results in a decrement in the observed CMB temperature. Unresolved galaxies, which together constitute the cosmic infrared background (CIB), on the other hand, appear as a diffuse background in the observed maps.  The tSZ and CIB signals on the sky will propagate through the quadratic estimator into the $\kappa_{\rm CMB}$ maps of \citetalias{Omori:2017}.  Since both non-Gaussian sources of contamination are correlated with the matter density, we also expect $\kappa_{\rm sys}$ to be correlated with the matter density. 

%There are several potential sources of systematic errors that could affect the measurement of $w^{\kcmb\gammat}(\theta)$. One useful diagnostic is to identify the list of external quantities that \textit{could} directly or indirectly contaminate the signal and cross-correlate them with the shear and the CMB convergence. We expect these cross-correlations to be consistent with zero if these external quantities are not introducing significant biases in the measurement. One example for such a quantity that could correlate both with shear and CMB convergence is dust extinction: since dust extinction is correlated with the galactic latitude, one would expect there to be fewer stars when there is high dust extinction, which could result in poor PSF modelling and biased shear estimates. On the other hand, dust is one of the foreground component of the CMB temperature measurements, and one can expect potential residuals in a single frequency temperature map. 

%We can test the impact of any potential systematic map $\mathcal{S}$ on our cross-correlation measurements by combining the correlations between all maps as follows. The observed cross-correlations $w^{\kcmb \delg}_{\mathrm{obs}}(\theta)$, which may be affected by contamination, are related to the underlying `true' correlations $w^{\kcmb\delg}_{\mathrm{true}}(\theta)$ by a correction term $w^{s}_{\mathrm{corr}}$ that depends on the systematic under consideration, and that can be written explicitly as $w^{s}_{\mathrm{corr}}(\theta) = w^{\kcmb \mathcal{S}}(\theta) w^{\delg\mathcal{S}}(\theta) / w^{\mathcal{S}\mathcal{S}}(\theta) $, so that \citep{CrocceACF}:
%\be
%w^{\kcmb \delg}_{\mathrm{obs}}(\theta) = w^{\kcmb \delg}_{\mathrm{true}}(\theta) + \frac{w^{\kcmb \mathcal{S}}(\theta) w^{\delg\mathcal{S}}(\theta)}{w^{\mathcal{S}\mathcal{S}}(\theta)} \, ,
%\label{eq:syscrosseq}
%\ee
%where $w^{\kcmb \mathcal{S}}(\theta), w^{\delg\mathcal{S}}(\theta), w^{\mathcal{S}\mathcal{S}}(\theta)$ are the correlation functions between the systematic map $\mathcal{S}$, the CMB lensing map, and the DES galaxy density map.
